EvalRS 2023. Well-Rounded Recommender Systems For Real-World Deployments

EvalRS aims to bring together practitioners from industry and academia to foster a debate on rounded evaluation of recommender systems, with a focus on real-world impact across a multitude of deployment scenarios. Recommender systems are often evaluated only through accuracy metrics, which fall short of fully characterizing their generalization capabilities and miss important aspects, such as fairness, bias, usefulness, informativeness. This workshop builds on the success of last year's workshop at CIKM, but with a broader scope and an interactive format.

==> src/activities.tex <==
\vspace{-1.0em}
\section{Format and Activities}\label{sec:activities}
% \wainline{Description of workshop activities. Outline how the workshop will be organized and how the time will be spent. In particular, please sketch how you will engage participants to foster more interactivity and engagement during the workshop.}
% \subsection{Tentative Schedule}
The duration of \textit{KaRS} would be \textbf{Half day}. The expected number of participants (based on the past editions) is $50$.

\noindent The tentative schedule for the workshop is organized as follows:
\begin{itemize}
    \item[09.00] Opening and Welcome
    \item[09.10] Invited Keynote
    \item[09.40] \textbf{Session I}
    \item[10.30] \textit{Break} 
    \item[11.00] \textbf{Session II}
    \item[12.10] Lessons learned and roundtable with the authors 
    \item[12.25] Wrap up and summary
\end{itemize}
The workshop will start with an invited Keynote. This will be followed by the first session of paper presentation. After the break, we will continue with a second session of papers. After the second session, we will summarize the advances in the field, and we will give the opportunity to the authors (and participants) to share ideas.

==> src/bios.tex <==
\section{Organizers}\label{sec:organizers}
% \wainline{
% Name, email address, and affiliation for workshop organizers and a brief description of their experience in organizing such events. Note that organizers are expected to attend the workshop and be actively involved in its organization.
% }
\noindent\textbf{Vito Walter Anelli}  (\href{mailto:vitowalter.anelli@poliba.it}{vitowalter.anelli@poliba.it}) is an Assistant Professor at Polytechnic University of Bari, affiliated with the Information Systems Laboratory (SisInf Lab). His current research interests fall in the areas of Recommender Systems, Knowledge representation, and User Modeling.
He has been awarded with the best research student paper at ISWC 2019~\cite{DBLP:conf/semweb/AnelliNSRT19}.
He has recently published a book chapter on interpretable RSs Systems~\cite{DBLP:series/ssw/AnelliBNS20}, and has published his works in international conferences, e.g., ECIR, RecSys, UMAP, SAC, ISWC, and ESWC; as well as in international journals, e.g., UMUAI, TKDE, and SWJ. Furthermore, he has served as chair of two international Workshops on Knowledge-aware Recommender Systems~\cite{DBLP:conf/cikm/AnelliN19,DBLP:conf/recsys/AnelliBBNLMNZ18}, RecSys 2021 challenge track, and RecSys 2020 challenge track~\cite{DBLP:conf/recsys/AnelliDSSABBGKL20}. 
His ORCID identifier is
 \url{https://orcid.org/0000-0002-5567-4307}.

\vspace{0.5em}
\noindent\textbf{Pierpaolo Basile} (\href{mailto:pierpaolo.basile@uniba.it}{pierpaolo.basile@uniba.it}) is Computer Science Assistant Professor (tenure-track position) at Universit\`a degli Studi di Bari Aldo Moro, Italy.
His main research interests are Natural Language Processing, Machine Learning for Natural Language Processing, Information Retrieval, Recommender Systems and Conversational Agents.
He authored several scientific papers published in international journals and collections, proceedings of international conferences and workshops, and book chapters. He organized several workshops in the area of Natural Language Processing, Information Retrieval and Recommender Systems. 
His ORCID identifier: \url{https://orcid.org/0000-0002-0545-1105}.

\vspace{0.5em}
\noindent\textbf{Tommaso Di Noia} (\href{mailto:tommaso.dinoia@poliba.it}{tommaso.dinoia@poliba.it}) is Professor of Computer Science at Polytechnic University of Bari. His research activities mainly focus on Artificial Intelligence and Data Management. He has been actively working in the field of recommender systems with many papers published in international journals, conferences, and book chapters. He has recently moved his research interests into the Trustworthy AI topic with a particular interest in adversarial machine learning, explainability, fairness, and privacy protection of recommendation models. His ORCID identifier is: \url{https://orcid.org/0000-0002-0939-5462}.

\vspace{0.5em}
\noindent\textbf{Francesco M.\ Donini} (\href{mailto:donini@unitus.it}{donini@unitus.it}) is Computer Science Professor at Universit\`a della Tuscia (Viterbo, Italy). His MAIN SCIENTIFIC INTERESTS are in Theory (Knowledge Representation in Artificial Intelligence; Algorithms and computational complexity of problems related to deduction in various logics) and in Applications (Intelligent Image retrieval, matchmaking in electronic marketplaces, negotiation, Semantic Web). His PUBLICATIONS amount to more than 100, and can be found through his ORCID identifier:
\url{https://orcid.org/0000-0003-0284-9625}.
SCIENTIFIC AWARDS On 1991 the paper "Tractable Concept Languages", (Int.\ Joint Conf.\ on Artificial Intelligence, IJCAI-91) received the Best Paper Award. On 2005 the paper "Concept Abduction and Contraction for Semantic-based Discovery of Matches and Negotiation Spaces in an E-Marketplace", (Int. Conf. on Electronic Commerce, ICEC-05) received the Best Paper Award. His SCIENTIFIC SERVICES include being PC CHAIR of the conferences: 1a) AICA-2002 (Conf.\ of the Italian Association for Informatics and Automated Calculus, Bari, Italy 2002) 1b) RDRC-06 (Resource Discovery Retrieval and Composition), Special Track of the ACM Symposium on Applied Computing (SAC), Dijon, France 2006; 1c) 1st Int.\ Worksh.\ on Semantic Matchmaking and Resource Retrieval: Issues and Perspectives" SMR 2006, Seoul, Korea - Sept.\ 11, 2006. He served as PC MEMBER in nearly all editions of the International Joint Conference on Artificial Intelligence (IJCAI) since 1993 (Blue Ribbon in 2019).

\vspace{0.5em}
\noindent\textbf{Cataldo Musto} (\href{mailto:cataldo.musto@uniba.it}{cataldo.musto@uniba.it}) is Assistant Professor at the Department of Informatics, University of Bari. His research is at the intersection of natural language processing, user modeling and recommender systems. Recent work focus on the analysis of fairness and explainability in intelligent information access systems. He organized several events related to user modeling and recommender systems, and he acts as program committee member in the main conferences of the area, such as ACM RecSys, ACM UMAP, ACM IUI and so on. Recently, he has also co-authored the book edited by Springer 'Semantics in Adaptive and Personalised Systems'. His ORCID identifier is: \url{https://orcid.org/0000-0001-6089-928X}. 

\vspace{0.5em}
\noindent\textbf{Fedelucio Narducci} (\href{mailto:fedelucio.narducci@poliba.it}{fedelucio.narducci@poliba.it}) is Assistant Professor (tenure-track position) at Polytechnic University of Bari, Italy. Over the years, he has authored several papers in international journals and conferences in the recommender-system research area. His current research interests include Recommender systems and machine learning, conversational agents, natural language processing, e-health, personalized information access, and user modeling and personalization. He has co-authored the book Semantics in Adaptive and Personalised Systems - Springer. His ORCID identifier is: \url{https://orcid.org/0000-0002-9255-3256}. 

\vspace{0.5em}
\noindent\textbf{Markus Zanker} (\href{mailto:markus.zanker@unibz.it}{markus.zanker@unibz.it}) is a professor at the Faculty of Computer Science of the Free University of Bozen-Bolzano, before moving to Bolzano he was an associate professor at the Alpen-Adria-Universitaet Klagenfurt, Austria. His research focuses on knowledge-based information systems supporting decision making processes such as personalized information filtering and retrieval and product recommendation. Until 2013 Markus Zanker was also a co-founder and director of a recommendation service company for more than 10 years. He is an associate editor of Information Technology \& Tourism (Springer) and of the recently launched ACM Transactions on Recommender Systems. Besides organizing numerous workshops in the field, he was a program chair of the 4th ACM Conference on Recommender Systems in 2010 and he co-chaired the 9th ACM Conference on Recommender Systems in 2015. His ORCID identifier is: \url{https://orcid.org/0000-0002-4805-5516}. 

==> src/bios_2022.tex <==
\section{Organizers}\label{sec:organizers}
% \wainline{
% Name, email address, and affiliation for workshop organizers and a brief description of their experience in organizing such events. Note that organizers are expected to attend the workshop and be actively involved in its organization.
% }
\noindent\textbf{Vito Walter Anelli}  (\href{mailto:vitowalter.anelli@poliba.it}{vitowalter.anelli@poliba.it}) is an Assistant Professor at Polytechnic University of Bari, affiliated with the Information Systems Laboratory (SisInf Lab). His current research interests fall in the areas of Recommender Systems, Knowledge representation, and User Modeling.
He has been awarded with the best research student paper at ISWC 2019~\cite{DBLP:conf/semweb/AnelliNSRT19}.
He has recently published a book chapter on interpretable RSs Systems~\cite{DBLP:series/ssw/AnelliBNS20}, and has published his works in international conferences, e.g., ECIR, RecSys, UMAP, SAC, ISWC, and ESWC; as well as in international journals, e.g., UMUAI, TKDE, and SWJ. Furthermore, he has served as chair of three international Workshops on Knowledge-aware Recommender Systems~\cite{DBLP:conf/cikm/AnelliN19,DBLP:conf/recsys/AnelliBBNLMNZ18}, RecSys 2021 challenge track, and RecSys 2020 challenge track~\cite{DBLP:conf/recsys/AnelliDSSABBGKL20}. 
His ORCID identifier is
 \url{https://orcid.org/0000-0002-5567-4307}.

\vspace{0.5em}
\noindent\textbf{Pierpaolo Basile} (\href{mailto:pierpaolo.basile@uniba.it}{pierpaolo.basile@uniba.it}) is Computer Science Associate Professor at Universit\`a degli Studi di Bari Aldo Moro, Italy.
His main research interests are Natural Language Processing, Machine Learning for Natural Language Processing, Information Retrieval, Recommender Systems and Conversational Agents.
He authored several scientific papers published in international journals and collections, proceedings of international conferences and workshops, and book chapters. He organized several workshops in the area of Natural Language Processing, Information Retrieval and Recommender Systems. 
His ORCID identifier: \url{https://orcid.org/0000-0002-0545-1105}.

\vspace{0.5em}
\noindent\textbf{Gerard de Melo} (\href{mailto:gerard.demelo@hpi.de}{gerard.demelo@hpi.de}) is a professor at the Hasso Plattner Institute for Digital Engineering and the University of Potsdam, Germany, where he leads the Artificial Intelligence and Intelligent Systems group. He has published over 150 papers on AI, natural language processing, knowledge graphs, and recommender systems, being awarded Best Paper awards at CIKM 2010, ICGL 2008, and the NAACL 2015 Workshop on Vector Space Modeling, among others. Previously, he was an assistant professor at Rutgers University in New Jersey and at Tsinghua University in Beijing, and a post-doctoral research scholar at ICSI/UC Berkeley. He received his doctoral degree at the Max Planck Institute for Informatics.
His ORCID identifier: \url{https://orcid.org/0000-0002-2930-2059}.

%\vspace{0.5em}
%\noindent\textbf{Tommaso Di Noia} (\href{mailto:tommaso.dinoia@poliba.it}{tommaso.dinoia@poliba.it}) is Professor of Computer Science at Polytechnic University of Bari. His research activities mainly focus on Artificial Intelligence and Data Management. He has been actively working in the field of recommender systems with many papers published in international journals, conferences, and book chapters. He has recently moved his research interests into the Trustworthy AI topic with a particular interest in adversarial machine learning, explainability, fairness, and privacy protection of recommendation models. His ORCID identifier is: \url{https://orcid.org/0000-0002-0939-5462}.

\vspace{0.5em}
\noindent\textbf{Francesco M.\ Donini} (\href{mailto:donini@unitus.it}{donini@unitus.it}) is Computer Science Professor at Universit\`a della Tuscia (Viterbo, Italy). His MAIN SCIENTIFIC INTERESTS are in Theory (Knowledge Representation in Artificial Intelligence; Algorithms and computational complexity of problems related to deduction in various logics) and in Applications (Intelligent Image retrieval, matchmaking in electronic marketplaces, negotiation, Semantic Web). His PUBLICATIONS amount to more than 100, and can be found through his ORCID identifier:
\url{https://orcid.org/0000-0003-0284-9625}.
SCIENTIFIC AWARDS On 1991 the paper "Tractable Concept Languages", (
%Int.\ Joint Conf.\ on Artificial Intelligence, 
IJCAI-91) received the Best Paper Award. On 2005 the paper "Concept Abduction and Contraction for Semantic-based Discovery of Matches and Negotiation Spaces in an E-Marketplace", (
%Int. Conf. on Electronic Commerce, 
ICEC-05) received the Best Paper Award. His SCIENTIFIC SERVICES include being PC CHAIR of the conferences: 1a) AICA-2002 
%(
%Conf.\ of the Italian Association for Informatics and Automated Calculus, Bari, Italy 2002) 
1b) RDRC-06
%(Resource Discovery Retrieval and Composition)
, Special Track of the ACM Symposium on Applied Computing (SAC), 
%Dijon, France 
2006; 1c) 1st Int.\ Worksh.\ on Semantic Matchmaking and Resource Retrieval: Issues and Perspectives" SMR 2006, Seoul, Korea - Sept.\ 11, 2006. He served as PC MEMBER in nearly all editions of 
%the International Joint Conference on Artificial Intelligence (
IJCAI 
%)
since 1993 (Blue Ribbon in 2019).

\vspace{0.5em}
\noindent\textbf{Antonio Ferrara} (\href{mailto:antonio.ferrara@poliba.it}{antonio.ferrara@poliba.it}) is a PhD and currently Assistant Researcher at Polytechnic University of Bari, affiliated with the Information Systems Laboratory (SisInf Lab). 
He mainly focuses on federated learning and its challenges ~\cite{Anelli2021_ecir}
%~\cite{DBLP:conf/aiia/AnelliDNF19}
, with a particular interest on its relevance for designing privacy-oriented RSs and building  knowledge-aware representations of user decision processes. Over the years, he published his works in national and international journals and presented full papers, demos, and tutorials at international conferences, including 
%SAC~\cite{DBLP:conf/sac/AnelliDNFN21}, ECIR~\cite{DBLP:conf/ecir/AnelliDNFN21},  
SIGIR~\cite{DBLP:conf/sigir/AnelliBFMMPDN21}, and RecSys~\cite{DBLP:conf/recsys/AnelliNSFM21,DBLP:conf/recsys/AnelliBFMMPDN21,DBLP:conf/recsys/AnelliBDNFNP21}. % He is a lecturer of AI and Computer Science academic courses.
He served as PC member and local organizer in international workshops, and as reviewer for international conferences and journals.
His ORCID identifier is \url{https://orcid.org/0000-0002-1921-8304}.


\vspace{0.5em}
\noindent\textbf{Cataldo Musto} (\href{mailto:cataldo.musto@uniba.it}{cataldo.musto@uniba.it}) is Assistant Professor (tenure-track position) at the Department of Informatics, University of Bari. His research is at the intersection of natural language processing, user modeling and recommender systems. Recent work focus on the analysis of fairness and explainability in intelligent information access systems. He organized several events related to user modeling and recommender systems, and he acts as program committee member in the main conferences of the area, such as ACM RecSys, ACM UMAP, ACM IUI and so on. Recently, he has also co-authored the book edited by Springer 'Semantics in Adaptive and Personalised Systems'. His ORCID identifier is: \url{https://orcid.org/0000-0001-6089-928X}. 

\vspace{0.5em}
\noindent\textbf{Fedelucio Narducci} (\href{mailto:fedelucio.narducci@poliba.it}{fedelucio.narducci@poliba.it}) is Assistant Professor (tenure-track position) at Polytechnic University of Bari, Italy. Over the years, he has authored several papers in international journals and conferences in the recommender-system research area. His current research interests include Recommender systems and machine learning, conversational agents, natural language processing, e-health, personalized information access, and user modeling and personalization. He has co-authored the book Semantics in Adaptive and Personalised Systems - Springer. His ORCID identifier is: \url{https://orcid.org/0000-0002-9255-3256}. 

\vspace{0.5em}
\noindent\textbf{Azzurra Ragone} (\href{mailto:azzurra.ragone@uniba.it}{azzurra.ragone@uniba.it}) is Assistant Professor (tenure-track position) at University of Bari Aldo Moro. Her current research interests fall in the areas of Trusted Artificial Intelligence, Recommender Systems, and Negotiation.
She worked as a researcher for several years at the Polytechnic of Bari, the University of Trento, the University of Michigan (USA) and the University of Milan Bicocca.
She also worked as Innovation and Transformation lead for EY, for Google as Program Manager, for BurdaForward as Branch Manager and for Exprivia S.p.A as a Project Manager and BI consultant for various Italian companies.
She has published her research works in more than 90 national and international workshops and conferences as well as in international journals.

\vspace{0.5em}
\noindent\textbf{Markus Zanker} (\href{mailto:markus.zanker@unibz.it}{markus.zanker@unibz.it}) is a professor at the Faculty of Computer Science of the Free University of Bozen-Bolzano, where he also served as vice dean for studies and director for study programmes. Before moving to Bolzano he was an associate professor at the Alpen-Adria-Universitaet Klagenfurt, Austria. His research focuses on knowledge-based information systems supporting decision making processes such as personalized information filtering and retrieval and product recommendation. Until 2013 Markus Zanker was also a co-founder and director of a recommendation service company for more than 10 years. He is an associate editor of Information Technology \& Tourism (Springer). Besides organizing numerous workshops in the field, he was a program chair of the 4th ACM Conference on Recommender Systems in 2010 and he co-chaired the 9th ACM Conference on Recommender Systems in 2015. His ORCID identifier is: \url{https://orcid.org/0000-0002-4805-5516}. 

\vspace{-1.0em}

==> src/dates_2022.tex <==

\subsection{Dates}
As suggested on the Call for Workshop, the important dates will be set as follows (deadlines refer to 23:59 -- 11:59pm -- in the AoE -- Anywhere on Earth -- time zone):
\begin{itemize}
\item Call for Papers publication: April 15th, 2022
\item Paper submissions due: August 5th, 2022
\item Paper acceptance notification: August 27th, 2022
\item Camera ready:	September 10th, 2022
\item Workshop day: September 18th, 2022
\end{itemize}
%Deadlines refer to 23:59 (11:59pm) in the AoE (Anywhere on Earth) time zone.
\vspace{-10px}

==> src/format.tex <==
\section{Format}\label{sec:format}
% \wainline{Requested duration (half day or full day), and expected number of participants.}
The duration of \textit{KaRS} would be \textbf{Half day}. The expected number of participants (based on the past editions) is $50$.

==> src/format_2022.tex <==

\section{Format and Activities}\label{sec:activities}
% \wainline{Description of workshop activities. Outline how the workshop will be organized and how the time will be spent. In particular, please sketch how you will engage participants to foster more interactivity and engagement during the workshop.}
% \subsection{Tentative Schedule}
The duration of \textit{KaRS} would be \textbf{Half day}. The format will be in person. expected number of participants (based on the past editions) is $50$.
The tentative schedule for the workshop is organized as follows:
\begin{itemize}
    \item[09.00] Opening and Welcome
    \item[09.10] Invited Keynote
    \item[09.40] \textbf{Session I}
    \item[10.30] \textit{Break} 
    \item[11.00] \textbf{Session II}
    \item[12.10] Lessons learned and roundtable with the authors 
    \item[12.25] Wrap up and summary
\end{itemize}
The workshop will start with an invited Keynote. This will be followed by the first session of paper presentation. After the break, we will continue with a second session of papers. After the second session, we will summarize the advances in the field, and we will give the opportunity to the authors (and participants) to share ideas.


==> src/prior_2022.tex <==
%\section{Dissemination of the results}\label{sec:dissemination}
% \wainline{Description of plans for promoting the workshop and disseminating the results, for instance, by organizing a journal special issue with extended versions of the workshop’s best papers.}
%We will distribute the workshop notes on the workshop website along with the video presentations, the slides, and the papers. 
%Video presentations and slides will be also disseminated on popular social media.
%Accepted papers will be also included in the workshop proceedings to be published on the CEUR-WS.org site or on the ACM Digital Library. 
%Authors of selected papers will be invited to contribute to a dedicated Special Issue.

\section{Related Workshops}\label{sec:priors}
% \wainline{History of prior workshops on this topic (e.g., including the number of submissions and attendees), if any.}

In this section, we briefly review the recent workshops (WSs) related to Knoweldge-aware and Conversational Systems.
\begin{itemize}[leftmargin=*]
 \item \textbf{1st, 2nd, and 3rd International Workshop on Knowledge-aware and Conversational Recommender Systems}\footnote{\url{https://kars-workshop.github.io/2018/}, \url{https://kars-workshop.github.io/2019/}, \url{https://kars-workshop.github.io/2021/}}.
These are the previous editions of the WS \cite{DBLP:conf/recsys/AnelliBBNLMNZ18,DBLP:conf/cikm/AnelliN19,DBLP:conf/recsys/AnelliBNDMNZ21}. 
%In 2021 @ RecSys, we received 15 submissions, 14 accepted; in 2019 (the workshop was hosted @ CIKM) 11 submissions, 6 accepted; and in 2018 @ RecSys, 12 submissions, 7 accepted.

    \item \textbf{3rd International Workshop on EntitY Retrieval and lEarning (EYRE 2020 @ CIKM)}\footnote{\url{https://sites.google.com/view/eyre20/home}}
This WS is focused on Entity Retrieval, which is substantially different from Recommender System. They are slightly related because also in EYRE structured data are exploited for Information Retrieval tasks.  

    \item \textbf{3rd International Workshop on ExplainAble Recommendation and Search (EARS 2020 @ SIGIR)}\footnote{\url{https://ears2020.github.io/}}
This WS is based on explainable recommendations. However, the focus is different because we promote the adoption of structured knowledge, and we cover also different topics as Conversational agents.

    \item \textbf{Joint Workshop on Bibliometric-enhanced Information Retrieval and Natural Language Processing for Digital Libraries (BIRDNL 2019)}\footnote{\url{http://www.sigir.org/sigir2019/program/workshops/birdnl/}}
The focus of this WS is on Digital Libraries. Structured knowledge and Information Retrieval are promoted, but the audience is not from Recommender Systems or Conversational Agents fields.

    \item \textbf{1st Workshop on Conversational Interaction Systems (WCIS 2019)}\footnote{\url{https://sites.google.com/view/wcis/home}}
This WS is only focused on Conversational Agents. In details, they focus more on speech recognition, spoken language understanding, language generation, and multi-modal question answering communities.

    \item \textbf{2nd International Workshop on Deep Learning on Graphs: Methods and Applications (DLG 2020 @ KDD)}\footnote{\url{https://deep-learning-graphs.bitbucket.io/dlg-kdd20/}}
The WS is related since they promote the adoption of deep learning techniques on graphs. However, Recommender systems, Conversational Agents and representations different from graphs are not considered.

    \item \textbf{Deep Learning for Knowledge Graphs (DL4KG 2020 @ ESWC)}\footnote{\url{https://alammehwish.github.io/dl4kg_eswc_2020/}}
This WS is related because they promote the adoption of deep learning techniques on graphs. However, Recommender systems and knowledge representations different from graphs are not considered.

    \item \textbf{6th Semantic Deep Learning (SemDeep-6 @ IJCAI-PRICAI 2020)}\footnote{\url{https://www.dfki.de/~declerck/semdeep-6/}}
The WS promote the adoption of Deep Learning techniques together with semantics. The focus of the WS is basically on (semi-automated) ontology learning, ontology alignment, ontology annotation, duplicate recognition, ontology prediction, knowledge base completion, relation extraction, and semantically grounded inference, which are topics that are very different from ours.

    \item \textbf{Explainable User Models and Personalized Systems (ExUM 2020 @ UMAP)}\footnote{\url{https://um.org/umap2020/attending/workshops-and-tutorials/}}
The WS focuses on Transparent Personalization Methods based on Heterogeneous and Personal Data. They cover the explainability of user modeling. However, Recommender Systems, Conversational Agents and structured knowledge representation are not considered.
\end{itemize}
%The above list of workshops co-located with top-tier conferences is clearly indicative of the importance of the proposed topic, and highlights to what extent RecSys can benefit from a workshop on Knoweldge-aware and Conversational Recommender Systems.

==> src/prior_workshops.tex <==
\section{History of prior workshops on this topic}\label{sec:priors}
% \wainline{History of prior workshops on this topic (e.g., including the number of submissions and attendees), if any.}

\noindent Workshops (WSs) on Knoweldge-aware and Conversational Systems in top-tier conferences.
\begin{itemize}
    \item \textbf{3rd International Workshop on EntitY Retrieval and lEarning (EYRE 2020 @ CIKM)}\footnote{\url{https://sites.google.com/view/eyre20/home}}
This WS is focused on Entity Retrieval, which is substantially different from Recommender System. They are slightly related because also in EYRE structured data are exploited for Information Retrieval tasks.  

    \item \textbf{3rd International Workshop on ExplainAble Recommendation and Search (EARS 2020 @ SIGIR)}\footnote{\url{https://ears2020.github.io/}}
This WS is based on explainable recommendations that are also covered by our proposal. However, the focus is different because we promote the adoption of structured knowledge, and we cover also different aspect as Conversational agents which make use of external knowledge.

    \item \textbf{Joint Workshop on Bibliometric-enhanced Information Retrieval and Natural Language Processing for Digital Libraries (BIRDNL 2019)}\footnote{\url{http://www.sigir.org/sigir2019/program/workshops/birdnl/}}
In this case, the focus of this WS is on Digital Libraries. Even though structured knowledge and Information Retrieval are promoted, the audience is not from Recommender Systems or Conversational Agents fields.

    \item \textbf{1st Workshop on Conversational Interaction Systems (WCIS 2019)}\footnote{\url{https://sites.google.com/view/wcis/home}}
This WS is only focused on Conversational Agents. In details, they focus more on speech recognition, spoken language understanding, language generation, and multi-modal question answering communities.

    \item \textbf{2nd International Workshop on Deep Learning on Graphs: Methods and Applications (DLG 2020 @ KDD)}\footnote{\url{https://deep-learning-graphs.bitbucket.io/dlg-kdd20/}}
The WS is related since they promote the adoption of deep learning techniques on graphs. However, Recommender systems, Conversational Agents and representations different from graphs are not considered.

    \item \textbf{Deep Learning for Knowledge Graphs (DL4KG 2020 @ ESWC)}\footnote{\url{https://alammehwish.github.io/dl4kg_eswc_2020/}}
This WS is related because they promote the adoption of deep learning techniques on graphs. However, Recommender systems and knowledge representations different from graphs are not considered.

    \item \textbf{6th Semantic Deep Learning (SemDeep-6 @ IJCAI-PRICAI 2020)}\footnote{\url{https://www.dfki.de/~declerck/semdeep-6/}}
This WS is related because they propose to adopt Deep Learning techniques together with semantics. However, the focus of the WS is basically on (semi-automated) ontology learning, ontology alignment, ontology annotation, duplicate recognition, ontology prediction, knowledge base completion, relation extraction, and semantically grounded inference, which are topics that are very different from ours.

    \item \textbf{Explainable User Models and Personalized Systems (ExUM 2020 @ UMAP)}\footnote{\url{https://um.org/umap2020/attending/workshops-and-tutorials/}}
This WS focuses on Transparent Personalization Methods based on Heterogeneous and Personal Data. It is related because they cover the explainability of user modeling. However, Recommender Systems, Conversational Agents and structured knowledge representation are not considered.
\end{itemize}
The above list of workshops co-located with top-tier conferences is clearly indicative of the importance of the proposed topic, and highlights to what extent RecSys can benefit from a workshop on Knoweldge-aware and Conversational Recommender Systems.

==> src/promotion_special_issue.tex <==
\section{Dissemination of the results}\label{sec:dissemination}
% \wainline{Description of plans for promoting the workshop and disseminating the results, for instance, by organizing a journal special issue with extended versions of the workshop’s best papers.}
We will distribute the workshop notes on the workshop website along with the video presentations, the slides, and the papers. 
Video presentations and slides will be also disseminated on popular social media.
Accepted papers will be also included in the workshop proceedings to be published on the CEUR-WS.org site or on the ACM Digital Library. 
Authors of selected papers will be invited to contribute to a dedicated Special Issue.

==> src/short_description.tex <==

% {\textcolor{red}{
% EVALUATION CRITERIA
% \begin{itemize}
%     \item Ability of the topic to contribute to the continued development of the field of recommender systems.
%     \item Level of complementarity of the topic to the main conference.
%     \item Clear plan for attracting submissions, making the workshop itself productive, and disseminating results.
%     \item Evidence that this plan will be successful.
%     \item Experience of the organizers.
% \end{itemize}
% }}

\section{Workshop Description}\label{sec:description}
% \wainline{
% % A short description of the workshop including the rationale for the workshop and how and why it fits the audience of RecSys. This description should include also the topic and its relevance to the community as well as format, and details about what type of submission is requested from prospective attendees. Please also add an explanation on how the workshop complements, rather than duplicates, the topics of the main conference.
% }
Recommender systems are becoming part of our daily life in many and diverse situations. Nevertheless, they start showing their limits in the tight interaction with human users~\cite{jannach2016recommender}. During the last years, owing in part to the new wave of deep learning approaches, a plethora of data-driven algorithms have been proposed that seek to identify latent connections among users and items~\cite{DBLP:journals/umuai/Fernandez-Tobias19,DBLP:conf/sigir/AnelliBFMMPDN21}. Despite their excellent results in terms of accuracy in recommending new items, such approaches very often miss a fundamental actor in the loop: the end-user. For this reason, current research is focusing on new challenges such as privacy \cite{DBLP:conf/recsys/AnelliBDNFNP21}, emotion awareness \cite{POLIGNANO2021114382}, and new paradigms such as federated learning \cite{Anelli2021_ecir,DBLP:conf/sac/AnelliDNFN21}. The exploitation of the knowledge about the domain of interest of a catalog via automated reasoning as well as critiquing approaches are very common in the normal behavior of a human user, but they are not well codified in recommendation engine behaviors. 
Knowledge-based approaches began to appear two decades ago~\cite{burke2000knowledge,DBLP:reference/sp/FelfernigFJZ15,zanker2010preference,DBLP:conf/semweb/AnelliNSRT19,DBLP:conf/recsys/AnelliNSFM21}. Nonetheless, they became more widely used with the advent of the Linking Open Data\footnote{\url{http://linkeddata.org}} initiative when a huge number of knowledge-graphs started being released and were made freely available. These include encyclopedic datasets such as DBpedia\footnote{\url{https://dbpedia.org}} and Wikidata\footnote{\url{https://wikidata.org}}, where semantics-aware information is available on different knowledge domains and applications~\cite{DBLP:conf/recsys/AnelliBFMMPDN21}. The exploitation of such datasets together with their ontologies is at the basis of many approaches to recommendation and challenges proposed in the last years such as Knowledge Graph embeddings~\cite{DBLP:journals/eswa/PalumboMRTB20,DBLP:conf/wsdm/ZhangXZZ20,DBLP:conf/www/NiLT20,DBLP:conf/aaai/DettmersMS018,DBLP:conf/esws/NayyeriVZY020}, hybrid recommendation~\cite{DBLP:conf/semweb/AnelliNSRT19,DBLP:conf/recsys/BelliniSNRS18a}, link prediction~\cite{DBLP:conf/www/HeLZLW20,DBLP:conf/www/0003W0HC19,DBLP:conf/aaai/DettmersMS018,DBLP:conf/esws/PiaoB18,DBLP:conf/esws/SchlichtkrullKB18,DBLP:conf/aaai/ShangTHBHZ19,DBLP:conf/kdd/Wang00LC19}, knowledge transfer~\cite{DBLP:journals/umuai/Fernandez-Tobias19}, interpretable recommendation~\cite{DBLP:conf/aaai/WangWX00C19,DBLP:journals/tkde/AnelliNSRT22,DBLP:conf/semweb/AnelliNSRT19}, and user modeling~\cite{DBLP:journals/tois/WangZWZLXG19,DBLP:journals/semweb/AnelliLNLR20,di2015recommender,DMMPR18}.
Successful workshops and international conferences in the last few years (ISWC, ACM Recommender Systems, UMAP, AAAI, ECAI, IJCAI, SIGIR) show the growing interest and research potential of these systems.

Furthermore, this side information associated with items becomes crucial when the interaction requires content features. This is the case of Conversational Recommender Systems (CRSs) \cite{zhou2020improving}.
CRSs are characterized by a multi-turn dialogue between the user and the system \cite{jannach2020survey} and are exploited in several domains \cite{Polignano2020}. Note that ``conversational'' as defined here is not restricted to CRSs that conduct dialogues in natural language. A CRS might converse in natural language, but it may allow more constrained modes of user interaction as well \cite{iovine2020conversational}. 
This kind of interaction introduces new challenges, since it blurs the difference between recommendation and retrieval. A CRS ought to be able to exploit both short- and long-term preferences, for example. Furthermore, a CRS should be able to adapt its behaviour in a timely manner when user feedback is provided. These are just some peculiarities of this kind of interaction. As we can imagine, another sensitive issue is the evaluation of CRSs \cite{zhang2020evaluating}, since also in this case we need to go beyond simple accuracy metrics. The limited availability of datasets is an additional obstacle to the evaluation of these systems \cite{iovine2019dataset}.
While research and development into CRSs has never gone away, it has certainly been less prominent for a while. 
Only recently has the literature on this topic been growing again quite notably~\cite{jannach2020survey}. 

%The topics addressed in this workshop are complementary to those of the main conference, in the sense that they focus the attention on peculiar aspects of conversational and knowledge-aware recommender systems. 
%Papers on preference elicitation through question-asking and on recommendation critiquing (\textit{like this but cheaper}) were common. While research and development into conversational recommenders has never gone away, it has certainly been less prominent for a while. 
%\vspace{-10px}

\subsection{Objectives}
The \textit{Fourth Knowledge-aware and Conversational Recommender Systems} (KaRS) Workshop focuses on all aspects related to the exploitation of external and explicit knowledge sources to feed and build a recommendation engine, and on the adoption of interactions based on the conversational paradigm. The aim is to go beyond the traditional accuracy goal~\cite{jannach2016recommender} and to start a new generation of algorithms and approaches with the help of the methodological diversity embodied in fields such as Machine Learning (ML), Human–Computer Interaction (HCI), Information Retrieval (IR), and Information Systems (IS). Hence, the focus lies on research improving the user experience and following goals such as user engagement and satisfaction or customer value as has also been advocated by Zanker et al.~\cite{zanker2019measuring}.
%which exploit the knowledge encoded in ontological and logic-based knowledge bases, knowledge graphs as well as the semantics emerging from the analysis of semi-structured textual sources. 
The aim of this fourth edition of KaRS~\cite{DBLP:conf/cikm/AnelliN19,DBLP:conf/recsys/AnelliBBNLMNZ18}
% , DBLP:conf/recsys/2018kars
is to bring together researchers and practitioners around the topics of designing and evaluating novel approaches for recommender systems in order to (i) share research and techniques, including new design technologies, (ii) identify next key challenges in the area, (iii) identify emerging topics in the field.
%\begin{itemize}
%	\item  share research and techniques, including new design technologies and evaluation methodologies;
%	\item identify next key challenges in the area;
%	\item identify emerging topics in the field.
%\end{itemize}
The workshop aims to establish an interdisciplinary community with a focus on the exploitation of \mbox{(semi-)structured} knowledge and conversational approaches for recommender systems and promoting collaboration opportunities.
%between researchers and practitioners.

\subsection{Topics}
Topics of interests include, but are not limited to:
{
%	\scriptsize
%\begin{itemize}
%\item{Knowledge-aware Recommender Systems}
\begin{itemize}[leftmargin=*]
    \item \textbf{Models and Feature Engineering}:
    Data models based on structured knowledge sources (e.g., Linked Open Data, Wikidata, BabelNet, etc.), Semantics-aware approaches exploiting the analysis of textual sources (e.g., Wikipedia, Social Web, etc.), Knowledge-aware user modeling, Methodological aspects (evaluation protocols, metrics, and datasets), Logic-based modeling of a recommendation process, Knowledge Representation and Automated Reasoning for recommendation engines, Deep learning methods to model semantic features
    \item \textbf{Beyond-Accuracy Recommendation Quality}: Using knowledge bases and knowledge graphs to increase recommendation quality (e.g., in terms of novelty, diversity, serendipity, or explainability), Explainable Recommender Systems, Knowledge-aware explanations (compliant with the General Data Protection Regulation)
    \item \textbf{Online Studies}: Knowledge sources for cross-lingual recommendations, Applications of knowledge-aware recommenders (e.g., music or news recommendation, off-mainstream application areas), User studies (e.g., on the user's perception of knowledge-based recommendations), field studies
    \item \textbf{Design of a Conversational Agent}: Design and implementation methodologies, Dialogue management (end-to-end, dialogue-state-tracker models), UX design, Dialogue protocol design
    \item \textbf{User Modeling and Interfaces}: Critiquing and user's feedback exploitation, Short- and Long-term user profiling and modeling, Preference elicitation, Natural language, multimodal, and voice-based interfaces, Next-question problem
    \item \textbf{Methodological and Theoretical aspects}: Evaluation and metrics, Datasets, Theoretical aspects of conversational recommender systems
\end{itemize}
%\end{itemize}
}

% SEZIONI COMMENTATE
%\input{src/bios_2022}
%\input{src/format_2022}
%\input{src/submissions_2022}
%\input{src/dates_2022}



%SEZIONI COMMENTATE
\input{src/prior_2022}

\section{Program Committee}\label{sec:committee}
The members of the Program Committee of KaRS 2022 are:
xxxxxxxxx



==> src/submission_and_pc.tex <==
\section{Submissions}\label{sec:submissions}
% \wainline{For workshops involving paper submissions, an initial -- and for the most part confirmed -- Program Committee (or a clear justification why it is not needed).}

We will invite three kinds of submissions, which address novel issues in Knowledge-aware and Conversational Recommender Systems: \begin{itemize}
    \item \textbf{Long Papers.} 
    \item \textbf{Short/Demo Papers.} 
    \item \textbf{Position/Discussion Papers.}
\end{itemize}
The short and long papers review process is \textbf{double-blind}. The authors must anonymize their submissions. Submitted papers will be evaluated according to their originality, technical content, style, clarity, and relevance to the workshop. Short and long paper submissions must be original work and may not be under submission to another venue at the time of review.
Accepted papers will appear in the \textbf{workshop proceedings}.

\subsection{Dates}
As suggested on the Call for Workshop, the important dates will be set as follow:
\begin{itemize}
\item Call for Papers publication: April 2nd, 2021
\item Paper submissions due: July 29th, 2021
\item Paper acceptance notification: August 14th, 2021
\item Camera ready:	September 4th, 2021
\item Workshop day: Oct 1st, 2021
\end{itemize}
Deadlines refer to 23:59 (11:59pm) in the AoE (Anywhere on Earth) time zone.

\section{Program Committee}\label{sec:committee}
Probable Program Committee based on past editions: 
\textbf{Dietmar Jannach} (Universität Klagenfurt)
% \textbf{Vito Walter Anelli} (Politecnico di Bari),
\textbf{Pablo Sánchez} (Universidad Autónoma de Madrid), \textbf{Phuong Nguyen} (Università degli Studi dell'Aquila), \textbf{Marijn Koolen} (Royal Netherlands Academy of Arts and Sciences - Humanities Cluster), \textbf{Iván Cantador} (Universidad Autónoma de Madrid), \textbf{Saikishore Kalloori} (ETH Zurich), \textbf{Adir Solomon} (Ben-Gurion University of the), \textbf{Bruce Ferwerda} (Jönköping University), \textbf{Anastasia Giachanou} (Universitat Politècnica de València), \textbf{Pablo Castells} (Universidad Autónoma de Madrid),
% \textbf{Tommaso Di Noia} (Polytechnic University of Bari),
\textbf{Mohammad Aliannejadi} (Università della Svizzera italiana (USI)),
% \textbf{Marco Polignano} (Università degli Studi di Bari Aldo Moro), \textbf{Salvatore Trani} (ISTI-CNR), \textbf{Ida Mele} (ISTI-CNR), \textbf{Alessandra Melonio} (Free University of Bozen-Bolzano), \textbf{Andrea Iovine} (Università degli Studi di Bari Aldo Moro), \textbf{Damiano Spina} (RMIT University), \textbf{Gaetano Rossiello} (University of Bari), \textbf{Marco Angelini} (Sapienza University of Rome), 
\textbf{Maurizio Ferrari Dacrema} (Politecnico di Milano),
% \textbf{Rosella Gennari} (Free U. of Bozen-Bolzano), \textbf{Pierpaolo Basile} (Dipartimento di Informatica - University of Bari), \textbf{Nicola Tonellotto} (), \textbf{Roberto Basili} (Dept. of Enterprise Engineering - Univ. of Roma Tor Vergata), 
\textbf{Alejandro Bellog\'in} (Universidad Autonoma de Madrid), 
% \textbf{Raffaele Perego} (ISTI-CNR), 
\textbf{Benjamin Heitmann} (RWTH Aachen University, Database and Information Systems Group (i5)), \textbf{Yashar Deldjoo} (Polytechnic University of Bari), \textbf{Derek Bridge} (University College Cork), 
% \textbf{Franco Maria Nardini} (ISTI-CNR), 
\textbf{Nourah Alrossais} (University of York), 
% \textbf{Maria Maistro} (University of Padua), \textbf{Danilo Croce} (Dept. of Enterprise Engineering - Univ. of Roma Tor Vergata), 
\textbf{Fabio Crestani} (University of Lugano (USI)), 
\textbf{Rubén Francisco Manrique} (Universidad de los Andes), \textbf{Nicola Ferro} (University of Padova), \textbf{Paolo Rosso} (Universitat Politècnica de València), \textbf{Olga Marino} (Universidad de los Andes), 
% \textbf{Giuseppe Amato} (ISTI-CNR), \textbf{Giorgiomaria Dinunzio} (), \textbf{Fedelucio Narducci} (University of Bari Aldo Moro), \textbf{Andrea Esuli} (Istituto di Scienza e Tecnologie dell'Informazione)

==> src/submissions_2022.tex <==

\section{Submissions}\label{sec:submissions}
% \wainline{For workshops involving paper submissions, an initial -- and for the most part confirmed -- Program Committee (or a clear justification why it is not needed).}

We will invite three kinds of submissions, which address novel issues in Knowledge-aware and Conversational Recommender Systems: \begin{itemize}
    \item \textbf{Long Papers.} 
    \item \textbf{Short/Demo Papers.} 
    \item \textbf{Position/Discussion Papers.}
\end{itemize}
The short and long papers review process is \textbf{double-blind}. 
%The authors must anonymize their submissions. 
Submitted papers will be evaluated according to their originality, technical content, style, clarity, and relevance to the workshop. Short and long paper submissions must be original work and may not be under submission to another venue at the time of review.
Accepted papers will appear in the \textbf{workshop proceedings}.

